Data-driven battery operation for energy arbitrage using rainbow deep reinforcement learning

As the world seeks to become more sustainable, intelligent solutions are needed to increase the penetration of renewable energy. In this paper, the model-free deep reinforcement learning algorithm Rainbow Deep Q-Networks is used to control a battery in a small microgrid to perform energy arbitrage and more efficiently utilise solar and wind energy sources. The grid operates with its own demand and renewable generation based on a dataset collected at Keele University, as well as using dynamic energy pricing from a real wholesale energy market. Four scenarios are tested including using demand and price forecasting produced with local weather data. The algorithm and its subcomponents are evaluated against two continuous control benchmarks with Rainbow able to outperform all other method. This research shows the importance of using the distributional approach for reinforcement learning when working with complex environments and reward functions, as well as how it can be used to visualise and contextualise the agent's behaviour for real-world applications.

==> algorithms/categorical.tex <==
\begin{algorithm}[t]
\caption{Categorical Algorithm}
\begin{algorithmic}[l]
\STATE Input transition $\langle s_t,a_t,r_t,s_{t+1} \rangle$
\STATE Calculate action-value of next state $Q(s_{t+1},a) = \sum_i z_i p_i (s_{t+1},a)$
\STATE Find next best action $a^{*} \leftarrow \argmax_a Q(s_{t+1},a)$
\STATE $m_i = 0$ with $i \in 0,\ldots, N_{\text{atoms}}-1$
\FOR{$j \in 0,\ldots, N_{\text{atoms}}-1$}
	\STATE $\mathcal{T}z_j \leftarrow [r_t+\gamma z_j]^{v_{\text{max}}}_{v_{\text{min}}} $
	\STATE $b_j \leftarrow (\mathcal{T}z_j - v_{\text{min}})/\Delta z$
	\STATE $l \leftarrow \lfloor b_j \rfloor $
	\STATE $u \leftarrow \lceil b_j \rceil$
	\STATE $m_l \leftarrow m_l + p_j (s_{t+1}, a^{*})(u - b_j) $
	\STATE $m_u \leftarrow m_u + p_j (s_{t+1}, a^{*})(b_j - l) $
\ENDFOR
\STATE
\end{algorithmic} \label{alg:cat}
\end{algorithm}

\begin{algorithm}[t]
\caption{Categorical Algorithm}
\begin{algorithmic}[l]
\STATE Input batch of transitions $\langle s_t,a_t,r_t,s_{t+1} \rangle$
\FOR{$i \in 0, \ldots, N_{\text{batch size}} $}
	\STATE Input transition $\langle s_t,a_t,r_t,s_{t+1} \rangle$
	\STATE Calculate action-value $Q(s_{t+1},a) = \sum_i z_i p_i (s_{t+1},a)$
	\STATE Find next best action $a^{*} \leftarrow \argmax_a Q(s_{t+1},a)$
	\STATE $m_j = 0$ with $j \in 0,\ldots, N_{\text{atoms}}-1$
	\FOR{$j \in 0,\ldots, N_{\text{atoms}}-1$}
		\STATE $\hat{\mathcal{T}}z_j \leftarrow [r_t+\gamma z_j]^{v_{\text{max}}}_{v_{\text{min}}} $
		\STATE $b_j \leftarrow (\mathcal{T}z_j - v_{\text{min}})/\Delta z$
		\STATE $l \leftarrow \lfloor b_j \rfloor $
		\STATE $u \leftarrow \lceil b_j \rceil$
		\STATE $m_l \leftarrow m_l + p_j (s_{t+1}, a^{*})(u - b_j) $
		\STATE $m_u \leftarrow m_u + p_j (s_{t+1}, a^{*})(b_j - l) $
	\ENDFOR
	\STATE $(\Phi \hat{\mathcal{T}} Z_{\hat{\theta}}(s,a))_i \leftarrow m $
\ENDFOR
\end{algorithmic} \label{alg:cat}
\end{algorithm}
